Taylor Genetic Programming for Symbolic Regression

Genetic programming (GP) is a commonly used approach to solve symbolic regression (SR) problems. Compared with the machine learning or deep learning methods that depend on the pre-defined model and the training dataset for solving SR problems, GP is more focused on finding the solution in a search space. Although GP has good performance on large-scale benchmarks, it randomly transforms individuals to search results without taking advantage of the characteristics of the dataset. So, the search process of GP is usually slow, and the final results could be unstable.To guide GP by these characteristics, we propose a new method for SR, called Taylor genetic programming (TaylorGP) (Code and appendix at https://kgae-cup.github.io/TaylorGP/). TaylorGP leverages a Taylor polynomial to approximate the symbolic equation that fits the dataset. It also utilizes the Taylor polynomial to extract the features of the symbolic equation: low order polynomial discrimination, variable separability, boundary, monotonic, and parity. GP is enhanced by these Taylor polynomial techniques. Experiments are conducted on three kinds of benchmarks: classical SR, machine learning, and physics. The experimental results show that TaylorGP not only has higher accuracy than the nine baseline methods, but also is faster in finding stable results.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> relatedworkbackup/relatedwork.tex <==
\section{Related Work}
\subsection{Machine learning for symbolic regression}
The regression analysis in machine learning, such as linear regression \cite{weisberg2005applied}, SVM \cite{cortes1995support}, XGBoost \cite{chen2016xgboost}, and neural network(NN) \cite{lecun2015deep}, is seen as a special case of SR. Different from SR that needs to find both the model and its parameter values, it is to find the values ($\theta$) of the parameters in a known model $f$, so that $f_{\theta}(X)=Y$. Owing to the known model $f$, it usually applies the gradient descent methods to obtain $\theta$. Nevertheless, handpicked neural networks can map the dataset $(X,Y)$ into a mathematical equation $f(X)=Y$ according to the features of the training dataset $\{(X,Y),\mathcal{F}\}$. 
% Most of these neural network utilizes an encoder-decoder architecture to implement the above mapping. 
GrammarVAE (GVAE) \cite{kusner2017grammar} trains a variational autoencoder \cite{kingma2013auto} to directly encode from and decode to the parse trees from a context-free grammar.
Recently, DSR \cite{petersen2021deep} has employed a recurrent neural network trained by the reinforcement learning based on a risk-seeking policy gradient to emit a distribution over tractable mathematical expressions. According to the distribution, DSR samples mathematical expressions with constant placeholders and obtain these constants by the nonlinear optimization algorithm -- BFGS \cite{fletcher2013practical}. 
Inspired by the recent successes of large pre-trained models on large datasets, such as BERT \cite{devlin-etal-2019-bert} and GPT \cite{brown2020language}, NeSymReS \cite{biggio2021neural} pre-trains the Set Transformer \cite{lee2019set} on hundreds of millions of equations to generate a distribution of mathematical expressions according to the given dataset $(X,Y)$. In addition, NeSymReS samples mathematical expressions with constant placeholders by the beam search on the distributions and uses BFGS to optimize these constants.

Besides the above neural networks for SR, EQL \cite{martius2016extrapolation,sahoo2018learning} designs a shallow fully-connected neural network where standard activation functions are replaced with basic functions (e.g., "$+$", "$\times$, "$sin$). Once the neural network is trained, it can represent a symbolic equation fitted to the given dataset. AIFeynman \cite{udrescu2020ai_a,udrescu2020ai_b} employs neural networks to map the given dataset into simplifying properties (e.g., symmetries, separability, and compositionality). It then designs a brute-force recursive algorithm guided by these simplifying properties and a suite of physics-inspired techniques to search all possible symbolic expressions. 

The above machine learning methods, especially deep learning methods, have the excellent ability to discover mathematical equations on some specific benchmarks. However, experiments on the large-scale benchmarks \cite{cava2021contemporary} indicate that the mathematical equations found by ML or DL are less accurate than those found by GP-based methods. For example, four of the top five methods and six of the top ten methods are GP-based methods, and the other top methods are ensemble tree-based methods, such as XGBoost and LightGBM \cite{ke2017lightgbm}. Surprisingly, the top methods do not include the two neural network methods, DSR and AIFeynman. Furthermore, the neural network methods seem to depend more on the training dataset.They can not discover a correct mathematical equation if the training dataset does not sufficiently cover the features of the given dataset.

\subsection{Genetic programming for symbolic regression}
% When Koza\cite{koza_genetic_1994} proposed GP, one of the goals of GP was to deal with SR.  
GP \cite{koza_genetic_1994} is a commonly used approach to deal with SR.
GP uses evolutionary operators\cite{forrest1993genetic} -- crossover, mutation, and selection, to change the individual encoding and generate better offspring for searching the mathematical expression space.
Various GPs employ different individual encodings to represent mathematical equations, such as tree-encoded GPs \cite{koza_genetic_1994,mckay_grammar-based_2010,hutchison_geometric_2012, trujillo2016neat, chen_improving_2019}, graph-encoded GPs \cite{CGP2008Miller,schmidt_distilling_2009}, and linearly encoded GPs \cite{ferreira2001gene,brameier2007linear}. 

For the mathematical expression space, the presence of real constants accounts for a significant portion of the size of the space. For example, the size of the aforementioned space in Section Introduction is $8.2\times 10^{162}$. Without real constants, the size of the space is $1.054\times 10^{19}$ \cite{korns2013baseline}. So, some GPs with a constant optimizer are propose to search the space, which they represent the skeleton of a mathematical expression by using constant placeholders and use a constant optimizer to find the values in these constant placeholders. AEG-GP \cite{korns2011accuracy,korns2013baseline} uses the abstract expression grammar to represent the skeleton of a mathematical expression and utilizes PSO \cite{kennedy1995particle} to find constant values. Different with AEG-GP, PGE \cite{worm2013prioritized} is an deterministic SR algorithm that offers reliable and reproducible results. While PGE maintains the tree-based representation and Pareto non-dominated sorting from GP, it replaces genetic operator and random number with grammar rules. It uses non-linear regression to fit the constants of an mathematical equation.  
The approaches to GP-based feature engineering, such as GP-based feature construction \cite{krawiec2002genetic}, MRGP \cite{arnaldo2014multiple}, FEW \cite{la2017general}, M3GP \cite{munoz2019evolving} and FEAT \cite{cava2018learning}, utilizes EC to search for possible representations and couple with an ML model to handle the parameters of the representations. For example, FEAT constructs a multi-type expression tree comprised of activation functions in neural networks (e.g., $tanh$, $sigmoid$, and $relu$) and basic functions (e.g., $+$,$-$, and $sin$) to represent a feature $\phi_i(x,\theta_i)$. It then linearly combines these features to show an individual, i.e., $y= \phi(x,\theta)^T\beta$, where $\phi=[\phi_1,...,\phi_k]$ and $\beta = [\beta_1,...,\beta_k]$. FEAT learns the weights ($\theta$) of the tree via stochastic gradient descent and fit the linear model by using ridge regression. FEAT uses a typical $\mu + \lambda$ evolutionary updating scheme to find the best data-fitted linear model. Different with GP-based feature engineering approaches, FFX \cite{mcconaghy2011ffx} is a deterministic SR algorithm. It enumerates a massive set of basic features (basis functions--$B_i(x)$) by a production rule. It then find coefficient values($a$) in $y=a_0+ \sum_{i=1}^{N} a_i \times B_i(x)$ by using pathwise regularized learning. 

All the above GPs search the mathematical expression space without considering the features of the given dataset. It means that they construct or change an individual without using the information of the give dataset. While these GP-based feature engineering approaches evaluate each feature (basic function) by the given dataset, they still do not use the information from the dataset to generate operators to transform these basic functions. Unlike these above GPs, semantic-based GPs can utilizes the dataset to transform individuals to search the space. The semantic of an individual $i$, $s(i)$, is the vector of $n$ numbers that $i$ returns when applied to the dataset. Geometric semantic GP(GSGP) \cite{hutchison_geometric_2012} creates the geometric crossover and mutation to generate an individual from its parent(s) in a way that guarantees to preserve their geometric properties. In this way, the mutated individual is semantically similar to the parent, and the crossover’s offspring has to be located on the segment between the semantics of the parents. Following the idea of the geometric operators in GSGP, many geometric operators, such as local geometric semantic crossover \cite{krawiec2013locally}, angle driven geometric semantic operators \cite{chen_improving_2019}, forward propagation mutation \cite{szubert2016semantic} and various semantic backpropagation operators \cite{krawiec2013approximating,pawlak2014semantic,virgolin2019linear}, are proposed to let GP execute the semantic search based on the given dataset. 

The other research line to guide GP by the features of the dataset is the hybrid of an neural network and a GP, called \textbf{DL-GP}. DL-GPs \cite{lu2016using,zhong2018deep,cranmer2020discovering,mundhenk2021symbolic,xing2021automated} handles an neural network to obtain features from the given dataset and applies these features to guide GP. For example, Xing, et al. \cite{xing2021automated} design a encoder-decoder neural network base on super-resolution ResNet to predicate the importance of each mathematical operator from the given data; and utilize the importance of each mathematical operator to guide GP. Cranmer, et al. \cite{cranmer2020discovering} train a graph neural network to represent sparse latent features of the given dataset, and employ GP to generate symbolic expressions fitted to these latent features. Mundhenk, et al. \cite{mundhenk2021symbolic} propose a hybrid neural-guide/GP approach to SR. The approach uses a RNN to generate N samples as the start population of a GP; and runs the GP with the start population to generate top M samples. It then trains the RNN with the M+N samples. After training the RNN, it again uses the RNN to generate N samples as the start population of the next-run GP. Repeat these steps until the hybrid approach find data-fitted symbolic equations. These above DL-GPs still depends on the time-consuming training work and the training dataset. 

Similar to AIFeynman, TaylorGP also need to extract the properties of the symbolic equation (e.g., separability and low-order polynomial ) from the given dataset. However, the different between them is that AIFeynman employ neural network to obtain these properties while TaylorGP achieves them by the coefficients in the Taylor series on the given dataset. So, TaylorGP do not need to train a model and not depend on the training data. Compared with semantic-based GP, TaylorGP do not need the complex semantic operators to generate individuals. Its operators are very simple.     

